Hydrodynamic equations and near critical large deviations of active lattice gases

Using a path integral approach, we derive and study the hydrodynamic equations and large deviation functions for three active lattice gases. After a review of the path integral for master equations, we first look at a one dimensional model of motility induced phase separation (MIPS), re-deriving the large deviation function that was previously found through a mapping to the ABC model. After extracting the deterministic hydrodynamic equations from the large deviation function, we analyse them perturbatively near the MIPS critical point using a weakly non-linear analysis. Doing this we show that they reduce to equilibrium Model B very close to criticality, with non-equilibrium, or Active Model B terms emerging as we leave the critical region. The same type of weakly non-linear analysis is then applied to the full large deviation function, and we show that the near critical stationary probability distribution is given by the exponential of a $\phi^4$ free energy, as expected in ordinary equilibrium phase separation. Similar calculations are then done for the two other lattice gases one which is another MIPS model, and another which models flocking, and in both cases we find analogous results.

==> code/quorum_phase_diagram <==
using Random, BenchmarkTools,Plots,LaTeXStrings
cd("/Users/lukeneville/Documents/PhD/current/hydro_path/figures/")

default(framestyle=:box,grid=false,
guidefont=font(12,"Computer Modern"),tickfont=font(12,"Computer Modern"),legendfont=font(10,"Computer Modern"),fg_legend = :transparent,dpi=300,
lw=2)

"""
Calculating the binodals by equality of h0 and g0 at the 
binodal densities.

r is related to the density via r=log(1-ρ)

Use newton's method
"""

function g0(r::Float64,p::Float64)
    p*log(r)/r +2*r/p
end

function h0(r::Float64,p::Float64)
    r^2/p +p*log(r)-(p/2)*(log(r))^2
end


function zerofunc(r10::Float64,r20::Float64,p::Float64)
    [g0(r10,p)-g0(r20,p),
    h0(r10,p)-h0(r20,p)]
end

function jacobian(r10::Float64,r20::Float64,p::Float64)
    jac=[(2/p +p/r10^2 -p*log(r10)/(r10^2))  -(2/p +p/r20^2 -p*log(r20)/(r20^2));
    (2*r10/p + p/r10 -p*log(r10)/r10)  -(2*r20/p + p/r20 -p*log(r20)/r20)]
    return jac
end


function g1(ρ::Float64,p::Float64)
   2*exp(ρ)/p + ρ*p*exp(-ρ)
end

function h1(ρ::Float64,p::Float64)
    exp(2*ρ)/p -ρ*p*(ρ-2)/2
end


function zerofunc1(ρ10::Float64,ρ20::Float64,p::Float64)
    [g1(ρ10,p)-g1(ρ20,p),
    h1(ρ10,p)-h1(ρ20,p)]
end

function jacobian1(ρ10::Float64,ρ20::Float64,p::Float64)
    jac=[(2*exp(ρ10)/p -p*(ρ10-1)*exp(-ρ10))  -(2*exp(ρ20)/p -p*(ρ20-1)*exp(-ρ20));
    (2*exp(2*ρ10)/p +p*(1-ρ10))  -(2*exp(2*ρ20)/p +p*(1-ρ20))]
    return inv(jac)
end


jacobian1(1.,2.,1.)

#Do newton's method to find the solution
#r10 and r20 are the initial guesses and pec is the peclet number 
#Returns the actual densities
function newton1(ρ10::Float64,ρ20::Float64,pec::Float64)
    ρ1n=copy(ρ10)
    ρ2n=copy(ρ20)
    for i in 1:100
        Δr=-jacobian1(ρ1n,ρ2n,pec)*zerofunc1(ρ1n,ρ2n,pec)
        ρ1n+=Δr[1]
        ρ2n+=Δr[2]
    end
    #return the R values
    return ρ1n,ρ2n
end




"""
Plotting Spinodals and binodals
"""

nx=400;
ρvals=LinRange(1.,2.5,nx);
ρval1=LinRange(.5,2.5,nx);
ρval2=LinRange(0.5,2.0,nx);
pecvals=LinRange(2*exp(3/2)*1.001,10.1,400);
rvals=(pecvals.-2*exp(3/2))./(2*exp(3/2));

binodals1=[]
binodals2=[]
pecsol=[]
for p in pecvals
    bins=newton1(1.0,2.0,p)
    push!(pecsol,p)
    push!(binodals1,bins[1])
    push!(binodals2,bins[2])
end


pushfirst!(binodals1,1.5)
pushfirst!(binodals2,1.5)
pushfirst!(pecsol,2*exp(3/2))

plot(binodals1,pecsol)

spin=sqrt(2)*exp.(ρvals)./sqrt.(ρvals.-ones(nx));
Plots.plot(binodals1,pecsol,lw=2,color=:red,fillrange=25,fillalpha=0.1,label="")
Plots.plot!(binodals2,pecsol,lw=2,color=:red,fillrange=25,fillalpha=0.1,label="")
Plots.plot!(ρvals,spin,fillrange=25,color=:lightskyblue2,fillalpha=1.0,label="",lw=:0,xlabel=L"\rho",ylabel="Pe",xlims=(0.95,2.2))
Plots.plot!(ρvals,spin,lw=2,color=:blue,ylims=(6,25),label="")



Plots.plot!(ρval1, 2*exp(3/2)*(1 .+((ρval1.-1.5).^2)./3.0),lw=2,color=:red,linestyle=:dash,label="")
Plots.plot!(ρval1, 2*exp(3/2)*(1 .+(2*(ρval1.-1.5).^2)./3.0),lw=2,color=:blue,linestyle=:dash,label="")
Plots.scatter!([1.5],[2*exp(3/2)],markersize=10,mc=:purple4,label="Critical Point",markerstrokecolor=:black,legend=:bottomleft)
annotate!(1.5, 18, "Spinodal Region",font(12,"Computer Modern"))


#savefig("quorum_phase_2.pdf")

==> hydro_path/FlockingGas.tex <==
\begin{tikzpicture}[scale=0.65]
\draw[-,color=BlueViolet,line width= .8mm] (0,0) -- (10.6,0);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,0) circle (.06);
\filldraw[color=Mahogany, fill=red!5,thick] (0.2,.4) circle (.2);

\filldraw[color=Blue, fill=blue!5,thick] (0.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (0.8,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (1.4,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (1.4,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] 
(2.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(2.6,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] 
(2.6,2.9) circle (.2);
\filldraw[color=Mahogany, fill=Red!5,thick] (3.2,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.2,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,2.2) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (5,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (5,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5,1.6) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (5.6,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.2,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (7.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (8.6,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (9.8,.4) circle (.2);
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,-4) circle (.06);
\draw [color=black!5,fill=black!5, smooth, samples=100, domain=0:10.6] plot(\x, {{sin(\x*25)*.3-2.5}}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen!5,fill=Green!20, smooth, samples=100, domain=0:10.6] plot(\x, {{sin(\x*20)*1.6-4}}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{{sin(\x*20)*1.6-4}});
\draw [color=black, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{{sin(\x*25)*.3-2.5}});
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\node[color=black] at (8.5,-2){$\rho(x)=\langle n^+ + n^-\rangle$};
\node[color=OliveGreen] at (2.3,-5){$m(x)=\langle n^+ - n^-\rangle$};
\draw[-to,color=Black, line width=.4mm] (9.8,.8) arc (130:70:.6);
\draw[-to,color=Black, line width=.4mm] (8.6,.8) arc (50:110:.6);
\draw[to-to,color=Black, line width=.4mm] (2.6,2) -- (2.6,2.6);
\filldraw[color=Blue, fill=blue!5,thick] (2.6,1.7) circle (.2);
\draw[-to,color=Black, line width=.4mm] (.4,.8) arc (50:110:.6);
\node at (0,1.5){$D+\lambda\ep$};
\node at (1.5,2.3){$\gamma\ep^2e^{-\beta}$};
\node at (8.6,1.4){$D+\lambda\ep$};
\node at (10,1.4){$D$};
\end{tikzpicture}

==> hydro_path/LatticeGas.tex <==
\begin{tikzpicture}[scale=0.65]
\draw[-,color=BlueViolet,line width= .8mm] (0,0) -- (10.6,0);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,0) circle (.06);
\filldraw[color=Blue, fill=blue!5,thick] (0.2,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (0.2,1) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (0.2,1.6) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (0.8,.4) circle (.2);
\filldraw[color=Blue,fill=blue!5,thick] (2,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (2.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (3.8,.4) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (4.4,.4) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (4.4,1) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (4.4,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (4.4,2.2) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (5,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (6.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (6.8,1) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (7.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (7.4,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8.6,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (9.2,.4) circle (.2);
\filldraw[color=Blue, fill=Blue!5,thick] (9.2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (9.2,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (10.4,.4) circle (.2);
\draw[-to,color=black, line width=.4mm] (10.4,.8) arc (130:70:.6);
\draw[-to,color=black, line width=.4mm] (.8,.8) arc (130:70:.6);
\draw[-to,color=black, line width=.4mm] (4.4,2.6) arc (70:130:.6);
\draw[-,color=BlueViolet,line width= .8mm] (0,-3) -- (10.6,-3);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,-3) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,-3) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,-3) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,-3) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,-3) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,-3) circle (.06);
\node at (.2,-2.5){$3$};
\node at (.8,-2.5){$1$};
\node at (1.4,-2.5){$0$};
\node at (2,-2.5){$2$};
\node at (2.6,-2.5){$1$};
\node at (3.2,-2.5){$0$};
\node at (3.8,-2.5){$1$};
\node at (4.4,-2.5){$4$};
\node at (5,-2.5){$1$};
\node at (5.6,-2.5){$0$};
\node at (6.2,-2.5){$0$};
\node at (6.8,-2.5){$2$};
\node at (7.4,-2.5){$2$};
\node at (8,-2.5){$1$};
\node at (8.6,-2.5){$2$};
\node at (9.2,-2.5){$3$};
\node at (9.8,-2.5){$0$};
\node at (10.4,-2.5){$1$};

\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,-6) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,-6) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,-6) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,-6) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,-6) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,-6) circle (.06);
\draw[-stealth,color=Black,line width=1mm] (10,-0.2) -- (10,-1.2);
\draw[-stealth,color=Black,line width=1mm] (10,-3.2) -- (10,-4.2);
\draw [color=blue!5,fill=blue!5, smooth, samples=100, domain=0:10.6] plot(\x, {cos(\x*80)*.3-sin(\x*50)*.4-4.5}) -- plot[domain=10.6:0] (\x, {-6}) -- cycle; 
\draw[-,color=BlueViolet,line width= .8mm] (0,-6) -- (10.6,-6);
\draw [color=Blue, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{cos(\x*80)*.3-sin(\x*50)*.4-4.5});
\draw[-to,color=Black,line width=0.3mm] (11,-5.8) -- (11,-4.2);
\node at (11.7,-5){$\rho(x)$};
\node at (11.5,-2.5){$n_i$};
\end{tikzpicture}

==> hydro_path/MIPSGas.tex <==
\begin{tikzpicture}[scale=0.65]
\filldraw[color=Blue, fill=blue!5,line width=0.4mm] (3,2.8) circle (.5);
\node[scale=2,color=Blue,line width= .8mm] at (3,2.8){$+$};
\draw[-to,color=Blue,line width=0.4mm] (3.5,2.8) -- (4.5,2.8);
\filldraw[color=Mahogany, fill=red!5,line width=0.4mm] (7.6,2.8) circle (.5);
\node[scale=2,color=Mahogany] at (7.6,2.8){$-$};
\draw[-to,color=Mahogany,line width=0.4mm] (7.1,2.8) --(6.1,2.8);
\draw[-,color=BlueViolet,line width= .8mm] (0,0) -- (10.6,0);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,0) circle (.06);
\filldraw[color=Blue, fill=blue!5,thick] (0.2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (0.8,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (3.2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (4.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (5,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5.6,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (7.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (8.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (9.8,.4) circle (.2);
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,-4) circle (.06);
\draw [color=Black!5,fill=Black!5, smooth, samples=100, domain=0:10.6] plot(\x, {cos(\x*40)*.3-sin(\x*120)*.4-1}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen!5,fill=OliveGreen!20, smooth, samples=100, domain=0:10.6] plot(\x, {-sin(\x*85)+sin(\x*120)*.4-4}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{-sin(\x*85)+sin(\x*120)*.4-4});
\draw [color=Black, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{{cos(\x*40)*.3-sin(\x*120)*.4-1}});
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\node[color=Black] at (8.2,-2){$\rho(x)=\langle n^+ + n^-\rangle$};
\node[color=OliveGreen] at (8.2,-5.2){$m(x)=\langle n^+ - n^-\rangle$};
\draw[-to,color=Black, line width=.4mm] (9.8,.8) arc (130:70:.6);
\draw[-to,color=Black, line width=.4mm] (4.4,.8) arc (50:110:.6);
\draw[to-to,color=Black, line width=.4mm] (.2,.8) arc (130:50:.6);
\draw[to-to,color=Black, line width=.4mm] (2.6,.8) -- (2.6,1.4);
\filldraw[color=Blue, fill=blue!5,thick] (2.6,1.7) circle (.2);
\node at (.5,1.4){$D$};
\node at (2,1.1){$\gamma\ep^2$};
\node at (4.5,1.4){$D+\lambda\ep$};
\node at (10,1.4){$D+\lambda\ep$};
\end{tikzpicture}

==> hydro_path/MIPSQuorum.tex <==
\begin{tikzpicture}[scale=0.65]
\draw[-,color=BlueViolet,line width= .8mm] (0,0) -- (10.6,0);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,0) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,0) circle (.06);
\filldraw[color=Blue, fill=blue!5,thick] (0.2,.4) circle (.2);

\filldraw[color=Blue, fill=blue!5,thick] (0.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (0.8,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (1.4,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (1.4,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] 
(2.6,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(2.6,1) circle (.2);
\filldraw[color=Mahogany, fill=Red!5,thick] (3.2,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.2,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(4.4,1.6) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,1) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] 
(3.8,1.6) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5,1.6) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5.6,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (5.6,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.2,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.2,1) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (6.8,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (7.4,.4) circle (.2);
\filldraw[color=Blue, fill=blue!5,thick] (8,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (8.6,.4) circle (.2);
\filldraw[color=Mahogany, fill=red!5,thick] (9.8,.4) circle (.2);
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.2,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.5,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (-0.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (10.8,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.1,-4) circle (.06);
\filldraw[color=BlueViolet, fill=BlueViolet,thick] (11.4,-4) circle (.06);
\draw [color=black!5,fill=black!5, smooth, samples=100, domain=0:10.6] plot(\x, {sin(\x*25)*.3-2}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen!5,fill=Green!20, smooth, samples=100, domain=0:10.6] plot(\x, {cos(\x*15)*2-4}) -- plot[domain=10.6:0] (\x, {-4}) -- cycle; 
\draw [color=OliveGreen, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{cos(\x*15)*2-4});
\draw [color=black, smooth, line width=0.3mm, samples=100, domain=0:10.6] plot(\x,{{sin(\x*25)*.3-2}});
\draw[-,color=BlueViolet,line width= .8mm] (0,-4) -- (10.6,-4);
\node[color=black] at (8.5,-3){$\rho(x)=\langle n^+ + n^-\rangle$};
\node[color=OliveGreen] at (2.3,-5){$m(x)=\langle n^+ - n^-\rangle$};
\draw[-to,color=Black, line width=.4mm] (5,2) arc (50:110:.6);
\draw[-to,color=Black, line width=.4mm] (.8,1.4) arc (130:70:.6);
\draw[-to,color=Black, line width=.4mm] (9.8,.8) arc (130:70:.6);
\node at (.8,1.8){$D+e^{-2\sigma_0}\lambda\ep$};
\node at (5,2.5){$D+e^{-3\sigma_0}\lambda\ep$};
\node at (9.8,1.2){$D$};
\end{tikzpicture}

==> hydro_path/fluctuationPath.tex <==
\begin{tikzpicture}[scale=0.6]
\draw[-stealth,color=gray,line width= .7mm] (0,-5) -- (0,5);
\draw[-stealth,color=gray,line width= .7mm] (-7,0) -- (7,0);
\node[scale=1.3] at (1,5){$\hat{\rho}$};
\node[scale=1.3] at (7,1){$\rho$};
\draw [color=Mahogany!5,fill=Mahogany!5, smooth, samples=100, domain=0:6] plot(\x, {-10*(\x/6)+10*(\x/6)^3}) -- plot[domain=6:0] (\x, {0}) -- cycle; 
\draw [color=Mahogany!5,fill=Mahogany!5, smooth, samples=100, domain=-6:0] plot(\x, {-10*(\x/6)+10*(\x/6)^3}) -- plot[domain=-6:0] (\x, {0}) -- cycle; 
\draw [-stealth, color=Mahogany, smooth, samples=100, domain=-6:-3,line width= .7mm] plot(\x,{-10*(\x/6)+10*(\x/6)^3});
\draw [color=Mahogany, smooth, samples=100, domain=-3:0,line width= .7mm] plot(\x,{-10*(\x/6)+10*(\x/6)^3});
\draw[-stealth, color=Blue, line width=0.7mm] (0,0)--(-3,0);
\draw[color=Blue, line width=0.7mm] (-2,0)--(-6,0);
\draw[-stealth, color=Blue, line width=0.7mm] (0,0)--(3,0);
\draw[color=Blue, line width=0.7mm] (2,0)--(6,0);
\node[scale=1] at (3.2,0.5){Deterministic};
\draw[decoration={
            text along path,
            text={Fluctuating},
            text align={center},
            raise=0.2cm},decorate] (-4.7,3) arc (155:25:1.5);
\draw [-stealth, color=Mahogany, smooth, samples=100, domain=6:3,line width= .7mm,] plot(\x,{-10*(\x/6)+10*(\x/6)^3});
\draw [color=Mahogany, smooth, samples=100, domain=3:0,line width= .7mm] plot(\x,{-10*(\x/6)+10*(\x/6)^3});
\filldraw[color=Black, fill=Black,thick] (0,0) circle (.2);
\filldraw[color=Black, fill=Black,thick] (-6,0) circle (.2);
\filldraw[color=Black, fill=Black,thick] (6,0) circle (.2);
\end{tikzpicture}
